Noisy Truncated SGD: Optimization and Generalization

Recent empirical work on stochastic gradient descent (SGD) applied to over-parameterized deep learning has shown that most gradient components over epochs are quite small. Inspired by such observations, we rigorously study properties of Truncated SGD (T-SGD), that truncates the majority of small gradient components to zeros. Considering non-convex optimization problems, we show that the convergence rate of T-SGD matches the order of vanilla SGD. We also establish the generalization error bound for T-SGD. Further, we propose Noisy Truncated SGD (NT-SGD), which adds Gaussian noise to the truncated gradients. We prove that NT-SGD has the same convergence rate as T-SGD for non-convex optimization problems. We demonstrate that with the help of noise, NT-SGD can provably escape from saddle points and requires less noise compared to previous related work. We also prove that NT-SGD achieves better generalization error bound compared to T-SGD because of the noise. Our generalization analysis is based on uniform stability and we show that additional noise in the gradient update can boost the stability. Our experiments on a variety of benchmark datasets (MNIST, Fashion-MNIST, CIFAR-10, and CIFAR-100) with various networks (VGG and ResNet) validate the theoretical properties of NT-SGD, i.e., NT-SGD matches the speed and accuracy of vanilla SGD while effectively working with sparse gradients, and can successfully escape poor local minima.

==> placeholder.tex <==
Consider the general setting that $\cA$ is a randomized algorithm and $S = \{z_1, ..., z_n\}$ be $n$ samples drawn i.i.d. from $\cP$. Denote $\cA(S)$ as the output of $\cA$ with the input to be $S$ and $\ell(\cA(S); z)$ denote the loss function of $\cA(S)$ applying to a sample $z$. 
The goal is to evaluate the population gradient
\begin{equation}
\nabla \mathcal{L}_{\mathcal{P}}(\mathcal{A}(S)) = \mathbb{E}_{z\sim \cP}[\nabla \ell(\mathcal{A}(S);z)]~. 
\end{equation}
Since $\cP$ is unknown, we can only measure the empirical gradient
\begin{equation}
\nabla \mathcal{L}_S(\mathcal{A}(S)) = \frac{1}{n}\sum_{z\in S}\nabla \ell(\mathcal{A}(S);z)~.
\end{equation}


We denote the generalization error as the difference between empirical gradient and population gradient
\begin{equation}
\text{err}_{\text {gen}}(\cA(S)) = \left\|\mathbb{E}_{S, \mathcal{A}} \nabla \mathcal{L}_{S}(\mathcal{A}(S))-\mathbb{E}_{S, \mathcal{A}} \nabla \mathcal{L}_{\mathcal{P}}(\mathcal{A}(S))\right\|~.
\end{equation}

With this notion of generalization error, we can bound the norm of the population gradient $\nabla \cL_{\cP}(\cA(S))$ with the norm of the empirical gradient and the generalization error
by triangle inequality and Jensen's inequality, i.e., 
\begin{equation} \label{eq:po_decom}
    \| \mathbb{E}_{S, \cA} \nabla \cL_{\cP}[\cA(S)]  \| \leq \mathbb{E}_{S, \cA} \| \nabla \cL_{S}[\cA(S)] \| + \text{err}_{\text {gen}}(\cA(S))~,
\end{equation}
where the first term in the right hand side of \eqref{eq:po_decom} refers to the optimization error which can be can be measured by the convergence rate of a iterative algorithm.

  

In order to bound the generalization error of an algorithm $\cA$, we employ the following notion of uniform stability which is inspired by the notion of uniform stability in \cite{hardt2016train,bousquet2002stability}. The key difference is that \cite{hardt2016train,bousquet2002stability} define the stability in terms of the loss function while we define the stability in terms of the norm of the gradient. 


\begin{defn}
[Uniform stability via the gradient] A randomized algorithm $\cA$ is $\alpha$-uniformly stable with respect to the gradient of the loss function $\ell$ if for all dataset $S, S^\prime \in \cZ^{n}$ such that $S$ and $S^\prime$  differ in at most one example, we have
\begin{equation}
\sup_{z} \mathbb{E}_{\cA}\left\|\nabla \ell(\cA(S); z)-\nabla \ell\left(\cA(S^\prime);z\right)\right\| \leq \alpha~.
\end{equation}
\end{defn}



Here, the expectation is taken only over the internal randomness of $\cA$. The algorithm $\cA$ can be any randomized algorithm. In the context of optimization, $\cA$ can be a gradient-based iterative algorithm that returns a parameter $\w = \cA(S)$ by minimizing the empirical risk. In this paper, $\cA$ is the NT-SGD algorithm and $\cA(S)$ is the parameter learnt by NT-SGD with training sample $S$. 




We recall the important argument that uniform stability implies generalization in expectation \citep{hardt2016train}. 
The following theorem shows that the norm of the difference between empirical gradient and population gradient can be bounded by the uniform stability $\alpha$. 


\begin{restatable}{theo}{theogen}
\textbf{(Generalization via uniform stability)}\label{theo:gen_stab}
Let $\cA$ be $\alpha$-uniformly stable with respect to the gradient. Then we have
\begin{equation}
    \left\| \mathbb{E}_{S, \cA} \nabla \cL_{S}(\cA(S)) -  \mathbb{E}_{S, \cA} \nabla \cL_{\cP}(\cA(S)) \right\| \leq \alpha~.
\end{equation}
\end{restatable}

With Theorem \ref{theo:gen_stab}, we can establish the bound for the population gradient $\nabla \cL_{\cP}(\cA(S))$ by triangle inequality and Jensen's inequality, i.e., 
\begin{equation} \label{eq:po_grad_bound}
    \| \mathbb{E}_{S, \cA} \nabla \cL_{\cP}[\cA(S)]  \| \leq \mathbb{E}_{S, \cA} \| \nabla \cL_{S}[\cA(S)] \| + \alpha~.
\end{equation}


With $\cA$ being NT-SGD for $T$ iterations and $\w_T = \cA(S)$ being the output of $\cA$ applied to training data $S$, we can quantify the population gradient $\|\mathbb{E}_{S, \cA} \nabla \cL_{\cP}(\w_T)\|$ by the norm of empirical gradient $\mathbb{E}_{S,\cA}\|\nabla \cL_{S}(\w_T)\|$ and the stability of NT-SGD. 
 
To establish the uniform stability of NT-SGD with $T$ iterations, we consider two datasets $S$ and $S^\prime$ that differ in at most one example. The goal is to bound $\sup_{z} \mathbb{E}\left\|\nabla \ell(\w_T); z)-\nabla \ell\left(\w_T^\prime);z\right)\right\|$ where $\w_T = \cA(S)$ and $\w_T^\prime = \cA(S')$ are respectively the outputs of NT-SGD with inputs $S$ and $S^\prime$. 
Since the gradient is $L$-Lipschitz, we have $\sup_{z} \mathbb{E}\left\|\nabla \ell(\w_T); z)-\nabla \ell\left(\w_T^\prime);z\right)\right\| \leq \sup_z L \mathbb{E} \|\w_T -\w_T^\prime \|$. Thus, the problem is reduced to bounding
$\mathbb{E}\|\w_T -\w_T^\prime \|$. We follow the gradient expansivity approach, first proposed by \cite{hardt2016train}, to show that $ \mathbb{E}\|\w_{t+1} -\w_{t+1}^\prime \|$ can be bounded by $ \mathbb{E}\|\w_{t} -\w_{t}^\prime \|$ with additional terms for any $t \leq T$ and applying the inequality recursively. 
Now we characterize the stability of NT-SGD with $T$ iterations in the following theorem. 








\begin{restatable}{theo}{theostab} \label{theo:stab}
Under Assumptions \ref{asmp: bounded_gradient} and \ref{asmp: zi_grad}, suppose that we run NT-SGD for $T$ iterations with batch size 
$|B_t| = m$, $\forall t \in [T]$, $\varepsilon \leq \frac{c^\prime}{n}$, $\sigma^2 = \frac{R}{p}$ for any $R \geq 0$, and $c^\prime > 0$. Then, we have

\hspace{2mm} 1. with step size $\eta_t = \frac{c}{t}$ for any $c > 0$, NT-SGD is $\alpha_T$-uniformly stable with
\begin{equation}
\alpha_{T} \leq O\left(\frac{G(m T)^{1 - \frac{1}{Lc +1}}}{n}\right).
% \frac{2G(2+c^\prime) (m T)^{1 - \frac{1}{Lc +1}}}{n(1-\frac{1}{n})}~.
\end{equation}

\hspace{2mm} \indent 2. with step size $\eta_t = \frac{c}{\sqrt{T}}$ for any $c > 0$, NT-SGD is $\alpha_T$-uniformly stable with
\begin{equation}
\alpha_{T} \leq O\left(\frac{GTm}{n}\right)~.
\end{equation}
\end{restatable}

Theorem \ref{theo:stab} shows 
presents bounds on the 
stability of NT-SGD for non-convex problems 
with two choices of step size, i.e.,  $\eta_t =c/t$ and $\eta_t = 1/\sqrt{T}$. With a smaller step size, i.e.,  $\eta_t =c/t$, the 
stability grows slower than the stability with a larger step size, i.e., $\eta_t = c/\sqrt{T}$.
For both choices of step sizes, the bounds increase as the batch size $m$ and the iteration number $T$ increase. When $\eta_t = c/\sqrt{T}$, the stability bound grows linearly with $T$. 
When $\eta_t = c/t$, the dependence on $n$ and $T$ in $\alpha_T$ of NT-SGD is the same as that in the stability bound of SGD (Theorem 3.12 in \cite{hardt2016train}) and Theorem \ref{theo:stab} matches the stability result of SGD  when $m = 1$. 
It is worth noting that, the stability decreases as $c$ decreases (step size $\eta$ decreases), e.g., 
\begin{enumerate}
    \item If $c = \frac{1}{L}$, $\alpha_T \leq O(\frac{\sqrt{T}}{n})$;
    \item If $c = \frac{1}{2L}$,  $\alpha_T \leq O(\frac{T^{1/3}}{n})$; 
    \item If $c=\frac{1}{9L}$,  $\alpha_T \leq O(\frac{T^{1/10}}{n})$. 
\end{enumerate}


There are other results on the stability of noisy SGD (SGLD) which follow the uniform stability notion proposed in \cite{hardt2016train}, i.e., in terms of the loss function. Recent work \citep{mou2018generalization,raginsky2017non,li2019generalization} have shown that the stability of SGLD can be bounded by the distance between the posterior distributions between running SGLD with $S$ and $S^\prime$, leading a $O(\frac{\sqrt{T}}{n})$ generalization bound in terms of the loss function. 

==> sections/convergence.tex <==
In this section, we establish the convergence rate of NT-SGD in terms of the norm of the empirical gradient.  

%\abcomment{maybe avoid using $R$, use $c_0$ or $\sigma_0$}

\begin{restatable}{theo}{theoopt}\label{theo:opt}
Under Assumptions \ref{asmp: bounded_gradient} and \ref{asmp: zi_grad}, for any $T >0$,  NT-SGD with $\eta_t = \eta = \frac{1}{\sqrt{T}}$, $\sigma^2 = \frac{R}{p}$ for any $R \geq 0$, $0\leq \varepsilon \leq \frac{\eta L}{2}$, we have
\begin{equation}
    %\frac{1}{T} \sum_{t=1}^{T} 
    \mathbb{E}\|  \nabla \cL_S(\w_J)\|^2 \leq O\left(\frac{L\left(G^2 + R^2)\right)}{\sqrt{T}}\right)
    % \frac{\cL_S \left(\mathbf{w}_{1}\right)-\cL_S^{\star}}{\sqrt{T}}+\frac{L\left(2G^2 + R^2)\right)}{\sqrt{T}},
\end{equation}
where $\mathbf{w}_{J}$ is uniformly sampled from $\left\{\mathbf{w}_{1}, \mathbf{w}_{2}, \ldots, \mathbf{w}_{T}\right\}$ produced by NT-SGD %\abcomment{what is the expectation over?}
and the expectation is over the randomness of NT-SGD and the random draw of $\w_J$.
%\abcomment{I am still confused -- so $R$ is an index over the iterations, and $w_R$ is the iterate at iteration $R$? and the variance increases with $R$ as $\sigma^2 = R/p$ -- this quite different from what I had in mind. Also, I dont quite understand the $w_R$ notation.}
\end{restatable}

Theorem \ref{theo:opt} shows that the convergence rate of NT-SGD is $O\left(\frac{1}{\sqrt{T}}\right)$ which matches the rate of SGD.
%and other gradient compression methods  \citep{signsgd,karimireddy2019error,Alistarh2018,quantized-sgd}. %Note that NT-SGD can be reduced to SGD when the cut rate $\varepsilon = 0$ and $R =0$. In that case, the bound in Theorem 1 characterizes the rate of SGD. 
When taking the cut rate $\varepsilon^2 = 0$ and $R =0$,  NT-SGD is reduced to SGD, and the bound in Theorem \ref{theo:opt} characterizes the rate of SGD. Proofs can be found in Appendix \ref{sec:app_opt}. 

